Scenarios and Recommendations for Ethical Interpretive AI

Artificially intelligent systems, given a set of non-trivial ethical rules to follow, will inevitably be faced with scenarios which call into question the scope of those rules. In such cases, human reasoners typically will engage in interpretive reasoning, where interpretive arguments are used to support or attack claims that some rule should be understood a certain way. Artificially intelligent reasoners, however, currently lack the ability to carry out human-like interpretive reasoning, and we argue that bridging this gulf is of tremendous importance to human-centered AI. In order to better understand how future artificial reasoners capable of human-like interpretive reasoning must be developed, we have collected a dataset of ethical rules, scenarios designed to invoke interpretive reasoning, and interpretations of those scenarios. We perform a qualitative analysis of our dataset, and summarize our findings in the form of practical recommendations.

==> learning.tex <==
\section{Learning}
\label{sec:learning}
%2-3 pages

In order to explore how well the dataset can be used to set benchmarks and train argument mining algorithms, two types of learning tasks were performed, which we describe next.

\subsection{Task 1: Predicting Individual Ratings}
\label{sec:task1}

Given a textual justification provided by a participant in Phase 2, can the numerical rating that user selected be predicted? All justifications were converted into 81,997-dimensional vectors consisting of three feature sets:

\begin{itemize}
    \item One-hot features for $n$-grams ($n = \{1,2,3\}$).
    \item The average of all Word2Vec vectors \cite{Mikolov2013a} corresponding to each word in the justification, ignoring OOV (out-of-vocabulary) words. Pre-trained Google News 300-dimensional vectors\footnote{\url{https://code.google.com/archive/p/word2vec/}} were used.
    \item Polarity and subjectivity of the justification, using TextBlob's sentiment analysis\footnote{\url{https://textblob.readthedocs.io/}} with default settings.
\end{itemize}
The above features were used to train several regression models: scikit-learn's\footnote{\url{https://scikit-learn.org/stable/}} ridge regression, random forest regression, and support vector machine regression, all with default parameters. All of these models were evaluated using 10-fold cross validation. Following \cite{Pavlick2016} (who also evaluated a dataset by training a model to predict human-labeled outputs on a five-point scale), the Spearman $\rho$ between the model's predictions and the actual human labels was calculated. Table \ref{tbl:task1_regression} reports the average Spearman $\rho$ for all 10 folds. 

\begin{table}[]
\begin{tabular}{|c|c|c|}
\hline
\textbf{Regression Model} & \textbf{Features} & \textbf{Avg $\rho$} \\
\hline
Ridge            & ngram                & 0.4054                           \\
\hline
Ridge            & W2V               & \textbf{0.4151}                           \\
\hline
Ridge            & Sentiment         & 0.09                             \\
\hline
Ridge            & All               & 0.4142                           \\
\hline
Random forest    & W2V               & 0.2272                           \\
\hline
Random forest    & All               & 0.3627                           \\
\hline
SVM             & W2V               & 0.3184                           \\
\hline
SVM              & All               & 0.4022                           \\
\hline
Random           & All               & 0.0169                          \\
\hline
\end{tabular}
\caption{Average Spearman $\rho$ over 10-fold cross-validation for Task 1. All p-values were under 0.001. Three feature sets (described in Section \ref{sec:task1}) were evaluated independently and together. Interestingly, using the Word2Vec vectors alone produced slightly better results with ridge regression, but this pattern did not repeat with other regression models.}
\label{tbl:task1_regression}
\end{table}

It is worth exploring whether the current task of predicting ratings given justifications is better conceived as a classification problem. Indeed, it is plausible that there is a qualitative difference between clear examples, clear non-examples, and ambiguous cases. Thus, we trained classification models using the feature sets described earlier. Three output labels were allowed, and assigned to the input data based on the rating: `negative' if the rating was 1, `ambiguous' if the rating was between 2 and 3, and `clear' if between 4 and 5---this division was chosen because it spread the corpus roughly evenly across the three labels.

Scikit-learn implementations of Gaussian Na\"{i}ve Bayes, linear SVM, and stochastic gradient descent were all used with default parameters. F-1 scores were calculated for each label over a 10-fold cross-validation, and the average F-1 scores are reported in Table \ref{tbl:task1_classification}.

\begin{table}[]
\begin{tabular}{|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Classification\\ Model\end{tabular}} & \textbf{F1 (W2V only)} & \textbf{F1 (All)} \\
\hline
Gaussian NB            & 0.4801            & 0.4727           \\
\hline
SGD                     & 0.5145           & \textbf{0.5753}   \\
\hline
SVM (linear)            & 0.5459           & 0.5747           \\
\hline
% SVM (radial)            &            & 0.2070            \\
% \hline
Random                  & \multicolumn{2}{c|}{0.3346}   \\
\hline
\end{tabular}
\caption{Average F-1 scores for feature sets consisting only of averaged Word2Vec vectors, and the full feature set described in Section \ref{sec:task1}.}
\label{tbl:task1_classification}
\end{table}


\begin{table*}[]
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Regression Model} & \textbf{Summary Features Only} & \textbf{Non-Summary Features Only} & \textbf{All Features} \\ \hline
Ridge & 0.05845 & \textbf{0.14261} & 0.13382 \\ \hline
Random Forest & -0.05231 & 0.11110 & 0.11932 \\ \hline
SVM & 0.03673 & 0.04581 & 0.08856 \\ \hline
Random & \multicolumn{3}{c|}{-0.01645} \\ \hline
\end{tabular}
\caption{Average Spearman $\rho$ over 10-fold cross-validation for Task 2. Feature sets are described in Section \ref{sec:task2}.}
\label{tbl:task2}
\end{table*}

\subsection{Task 2: Predicting Average Ratings}
\label{sec:task2}

A more difficult task is to actually determine the applicability of a phrase to a scenario. More precisely: Given a rule, phrase, and scenario, can it be determined whether the scenario is (1) a clear instance of the phrase as used in the rule, (2) a clear non-example of the phrase as used in the rule, or (3) an ambiguous example of the phrase as used in the rule? The average ratings per scenario provided by our dataset provide an approximation of this that we can train a model to predict.

In practice, we expect this to be a very difficult task for current AI systems. It would seem that determining whether a scenario can be interpreted as an instance of a given phrase would require, at a minimum, the ability to generate a wide variety of interpretive arguments for and against, and then assess that group of interpretive arguments as a whole. Indeed, the level of disagreement between individual raters in our dataset suggests that this is even a difficult problem for individual humans---the ambiguity of a phrase may only become apparent when competing arguments are made explicit. 

Nevertheless, it is useful to set a benchmark against which future models can compare. We trained regression models to predict the average rating given to a scenario, using the following feature set:

\begin{itemize}
    \item One-hot features for $n$-grams ($n = \{1,2,3\}$). Only the phrase was used, as initial testing showed that including additional text (e.g., the rule or scenario description) had detrimental effects.
    \item Averaged Word2Vec vectors, as in Task 1. The average vectors for the rule, phrase, and scenario description were calculated and concatenated.
    \item Polarity and subjectivity of the phrase and scenario description.
    \item Textual entailment features.
    \item Doc2Vec distances.
\end{itemize}
To calculate textual entailment features, we used a single LSTM layer\footnote{We used the implementation at \url{https://www.oreilly.com/learning/textual-entailment-with-tensorflow}.} trained on the full Stanford NLI training set \cite{Bowman2015}. Training was performed over 500,000 iterations, yielding a final training accuracy of 63.3\%. When this training was complete, four combinations of inputs were fed into the network as premise / conclusion: rule / scenario description, scenario description / rule, phrase / scenario description, and scenario description / phrase. For each of these combinations, the textual entailment network produced four outputs, each of which were used as features: a confidence that the premise / conclusion pair constitutes a positive, negative, or neutral inference, and an integer reflecting which of these confidence values was highest: -1, 0, or 1 depending on if the highest confidence was neutral, negative, or positive, respectively.

Doc2Vec distances were included to attempt to capture semantic overlap. All rules, phrases, and scenario descriptions were used to train the Doc2Vec model \cite{Le2014}, and then were all converted into 300-dimensional Doc2Vec vectors. After conversion to vectors, both the cosine distance and Euclidean distance between phrases and their corresponding scenario descriptions, and between rules and their scenario descriptions, were added as features.

Three regression models were trained on three combinations of features: summary features only (consisting of all features above except for the one-hot and Word2Vec vectors), non-summary features only (one-hot and Word2Vec vectors), and all features. Unfortunately, the results, listed in Table \ref{tbl:task2}, are only barely above the random baseline, and did not have significant p-values. 
